Multi-Agent Transfer Learning in Reinforcement Learning-Based Ride-Sharing Systems

Reinforcement learning (RL) has been used in a range of simulated real-world tasks, e.g., sensor coordination, traffic light control, and on-demand mobility services. However, real world deployments are rare, as RL struggles with dynamic nature of real world environments, requiring time for learning a task and adapting to changes in the environment. Transfer Learning (TL) can help lower these adaptation times. In particular, there is a significant potential of applying TL in multi-agent RL systems, where multiple agents can share knowledge with each other, as well as with new agents that join the system. To obtain the most from inter-agent transfer, transfer roles (i.e., determining which agents act as sources and which as targets), as well as relevant transfer content parameters (e.g., transfer size) should be selected dynamically in each particular situation. As a first step towards fully dynamic transfers, in this paper we investigate the impact of TL transfer parameters with fixed source and target roles. Specifically, we label every agent-environment interaction with agent's epistemic confidence, and we filter the shared examples using varying threshold levels and sample sizes. We investigate impact of these parameters in two scenarios, a standard predator-prey RL benchmark and a simulation of a ride-sharing system with 200 vehicle agents and 10,000 ride-requests.

==> section/relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}
This section briefly reviews recent work that apply transfer learning in simulated environment for mobility on-Demand applications.

%RS ADDRESSED BY RL
Within the literature, to address the rider-driver matching problem in mobility on-Demand systems, are available a wide range of techniques, using different inputs and assumptions.
A complete review of these techniques is out of scope for this work, however we could categorized in centralized and decentralized.
Generally, the former aims to optimize the overall performance, i.e., minimising the travelled distance~\cite{yang2019, Fagnant2017, Wen2017} while the latter, addresses the problem from a single vehicle perspective where each vehicle is independent and unaware of others doing.
Decentralized approaches often relies on reinforcement learning where each vehicle is controlled by a single agent~\cite{castagna2020d2r2, castagna2020demand, samod2020,alabbasi2019deeppool}.

In this paper, we adopt a decentralized version from our previous work~\cite{castagna2020d2r2}, here we disable the rebalancing scheduler and replace the underlying engine with a widely adopted simulator of urban mobility, SUMO~\cite{sumo2018}. 

\textbf{\title{Transfer Learning in rider-driver Assignment}}

%TRANSFER LEARNING IN RIDER-DRIVER ASSIGNMENT
Within rider-driver dispatch problem there are not many works that bootstrap external knowledge applying transfer learning.

Previously, in~\cite{castagna2020d2r2,castagna2020demand}, we designed a multi-agent collaborative algorithm to obtain a main knowledge that is then replicated to other agents. In detail, multiple agents were learning to satisfy ride-requests in a iterative way where the set of available requests was composed by unserved requests from previous vehicles.
Finally, obtained knowledge is replicated to any other agent that is joining the fleet and no further refinement steps are performed.

On the other hand, ~\cite{wang2018smartcity,wang2018DRLknowledgetransfer}, bootstrap previous acquired knowledge with a fine-tuning process to leverage a pre-trained learning model.
Here, authors use a deep learning model and transfer a pre-trained neural network to target environments with different demand pattern and road infrastructure.
This technique limits the range of applicable algorithms to those with a neural network underlying as it is feasible to transfer just the layers weights, i.e., is not possible to transfer knowledge to tabular model. Furthermore, any change in the neural network architecture require further steps to adapt the pre-trained layers.


\cite{wan2021pattern} proposes an approach to transfer from source to a target environment. The goal is to fine-tune knowledge by adapting the source value-function to a target task with a concordance penalty that expresses the similar patterns between the two tasks, i.e. demand pattern.
Thus, it can be applied to a range of rl techniques regardless the underlying representation. Nevertheless, a strong limitation of this work is the need of prior knowledge over the relation between source and target tasks.


\begin{comment}
epsitemic confidence level of the agent the RND work + multi-heads nn

reusing experience from one to other with other polocies, i.e., latest episodes...
\end{comment}

%todo want to say:  (1) learning from demonstrator (2) tl+ mistake correction; (3) fine tuning


